InPL: Pseudo-labeling the Inliers First for Imbalanced Semi-supervised Learning

Recent state-of-the-art methods in imbalanced semi-supervised learning (SSL) rely on confidence-based pseudo-labeling with consistency regularization. To obtain high-quality pseudo-labels, a high confidence threshold is typically adopted. However, it has been shown that softmax-based confidence scores in deep networks can be arbitrarily high for samples far from the training data, and thus, the pseudo-labels for even high-confidence unlabeled samples may still be unreliable. In this work, we present a new perspective of pseudo-labeling for imbalanced SSL. Without relying on model confidence, we propose to measure whether an unlabeled sample is likely to be ``in-distribution''; i.e., close to the current training data. To decide whether an unlabeled sample is ``in-distribution'' or ``out-of-distribution'', we adopt the energy score from out-of-distribution detection literature. As training progresses and more unlabeled samples become in-distribution and contribute to training, the combined labeled and pseudo-labeled data can better approximate the true class distribution to improve the model. Experiments demonstrate that our energy-based pseudo-labeling method, \textbf{InPL}, albeit conceptually simple, significantly outperforms confidence-based methods on imbalanced SSL benchmarks. For example, it produces around 3\% absolute accuracy improvement on CIFAR10-LT. When combined with state-of-the-art long-tailed SSL methods, further improvements are attained. In particular, in one of the most challenging scenarios, InPL achieves a 6.9\% accuracy improvement over the best competitor.

==> figures/visualization.tex <==
\begin{figure}[t]
\centering
\subfloat[Energy-based Pseudo-label Decision]{%
  \includegraphics[width=\linewidth]{pics/energy_vis.pdf}%
  \label{fig:cifar_thres}%
}\qquad
\subfloat[Confidence-based Pseudo-label Decision]{%
  \includegraphics[width=\linewidth]{pics/confidence_vis.pdf}%
  \label{fig:cifar_lt_thres}%
}\qquad
\caption{\textbf{Visualization: energy score vs confidence score}: The shaded region denotes the which data points are pseudo-labeled. (a) Energy-based Pseudo-Label Decision and (b) Confidence-based Pseudo-Label Decision. Notice that energy-based pseudo-labelling produces correct pseudo-labels for many low-confident unlabeled examples.}
\label{fig:visualization}
\end{figure}

==> tables/baseline_app.tex <==
\begin{table}
  \begin{tabular}{lcc}
    \toprule
        & CIFAR10 $N=40$ & SVHN $N=40$ \\ 
        \cmidrule(l{3pt}r{3pt}){2-3} 
    FixMatch~\cite{sohn2020fixmatch}     & 92.53{\scriptsize $\pm$0.28} & 96.19{\scriptsize $\pm$1.18} \\
    FixMatch-UPS~\cite{rizve2021defense} & 93.74{\scriptsize $\pm$0.87} & 97.20{\scriptsize $\pm$0.17} \\
    FixMatch-ABC~\cite{lee2021abc} & 93.16{\scriptsize $\pm$0.29} & 95.24{\scriptsize $\pm$1.64} \\
    EnergyMatch (ours) &  \textbf{94.58}{\scriptsize $\pm$0.43} & \textbf{97.78}{\scriptsize $\pm$0.05} \\
        \bottomrule
    \end{tabular}
      \caption{Comparison to FixMatch-UPS and FixMatch-ABC on CIFAR10 and SVHN with 40 labeled data in total (balanced setting).}%
  \label{tab:baseline_app}

\end{table}

==> tables/hyper.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \caption{Hyper-parameter and training details for results in Table 1 and Table 3. All experiments use the same set of learning rate, loss weight, batch size, and EMA momentum.}
    \begin{adjustbox}{width=0.87\columnwidth,center}
    \begin{tabular}{ccccccc}
    \toprule
  Hyper-parameter & CIFAR10 & SVHN  & STL10 & CIFAR100 & CIFAR10-LT & CIFAR100-LT \\ 
  \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  Energy Threshold &  -8.0 & -8.0 & -8.0 & -11.0 & -9.5 & -12.5 \\
  \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  Weight Decay & 0.0005 & 0.0005 & 0.0005 & 0.001 & 0.0005 & 0.001 \\
  \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  Learning Rate & 0.03 & 0.03 & 0.03 & 0.03 & 0.03 & 0.03 \\
  Weight of Unsupervised Loss & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
  Labeled Batch Size & 64 & 64 & 64 & 64 & 64 & 64 \\
  Unlabeled Batch Size & 448 & 448 & 448 & 448 & 448 & 448 \\
  EMA momentum & 0.999 & 0.999 & 0.999 & 0.999 & 0.999 & 0.999 \\

  \bottomrule
  
  \end{tabular}
    \end{adjustbox}
    
    \label{tab:hyper}
\end{table}

==> tables/realistic.tex <==
\begin{figure}
\label{fig:realistic}
\begin{floatrow}
\ffigbox{%
  \includegraphics[width=.55\linewidth]{pics/precision_body.pdf}
}{%
  \caption{A figure}%
}
\begin{adjustbox}{width=0.45\columnwidth}
\capbtabbox{%
  \begin{tabular}{lcccc}
    \toprule
   & Labeled Set & Unlabeled Set  & Accuracy \\ 
   \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-4}
  FixMatch~\cite{sohn2020fixmatch} & \multirow{ 3}{*}{CIFAR10} & \multirow{ 3}{*}{CIFAR10 + SVHN} & 62.60 \\
  FlexMatch~\cite{zhang2021flexmatch} & & & 60.03 \\
  EnergyMatch & & & \textbf{67.02} \\
  
  \hline
  \end{tabular}
}{%
  \caption{A table}%
}
\end{adjustbox}
\end{floatrow}
\end{figure}
